Gaia Data Release 3: Cross-match of Gaia sources with variable objects from the literature

Context. In the current ever increasing data volumes of astronomical surveys, automated methods are essential. Objects of known classes from the literature are necessary for training supervised machine learning algorithms, as well as for verification/validation of their results. Aims.The primary goal of this work is to provide a comprehensive data set of known variable objects from the literature cross-matched with \textit{Gaia}~DR3 sources, including a large number of both variability types and representatives, in order to cover as much as possible sky regions and magnitude ranges relevant to each class. In addition, non-variable objects from selected surveys are targeted to probe their variability in \textit{Gaia} and possible use as standards. This data set can be the base for a training set applicable in variability detection, classification, and validation. MethodsA statistical method that employed both astrometry (position and proper motion) and photometry (mean magnitude) was applied to selected literature catalogues in order to identify the correct counterparts of the known objects in the \textit{Gaia} data. The cross-match strategy was adapted to the properties of each catalogue and the verification of results excluded dubious matches. Results.Our catalogue gathers 7\,841\,723 \textit{Gaia} sources among which 1.2~million non-variable objects and 1.7~million galaxies, in addition to 4.9~million variable sources representing over 100~variability (sub)types. Conclusions.This data set served the requirements of \textit{Gaia}'s variability pipeline for its third data release (DR3), from classifier training to result validation, and it is expected to be a useful resource for the scientific community that is interested in the analysis of variability in the \textit{Gaia} data and other surveys.

==> DPACP-177_GAIA Cross-match/EB_naming_conv_table.tex <==

\begin{table}
\caption{\label{table:eb_naming_conv} Convention between different classes and sub-classes of eclipsing binaries and how they merged to 4 generic classes, ECL, EA, EB, and EW.}
\centering
\begin{tabular}{lllll}
\hline
\hline
\multicolumn{5}{c}{EA}\\
\hline
BETA\_PERSEI&detached&detachedEB&E/D &E/D/WR \\
E/DM&E/DS&E/DW & EA &EA/AR\\
EA/AR/RS&EA/AR: &EA/D &EA/D/R&EA/D/RS\\
EA/D/WR &EA/D:&EA/DM&EA/DM/RS&EA/DM: \\ 
EA/DS &EA/DS/RS&EA/DS:&EA/DW & EA/DW/RS \\
EA/GS&EA/GS+ &EA/GS/D &EA/GS/RS & EA/HW\\
EA/K&EA/KE &EA/KE: &EA/KW & EA/PN\\
EA/RS &EA/RS: &EA/WD&EA/WD/RS& EA/WR \\
EB\_ED&ECL/NC &ECLED&ECLNC & ED \\ 
NC&NONEC& \\
\multicolumn{5}{c}{}\\
\hline
\hline
\multicolumn{5}{c}{EB}\\
\hline
BETA\_LYRAE&E/SD&EB&EB/A & EB/AR/RS\\
EB/D&EB/D/G&EB/D/GS & EB/D:&EB/DM\\
EB/DM/WR&EB/DM: &EB/DS&EB/DW&EB/DW/RS\\
EB/GS &EB/GS/D&EB/RS&EB/SD&EB/SD: \\ 
EB/WR&EB\_ESD&ESD&near\_contac & semi-detached \\
\multicolumn{5}{c}{}\\
\hline
\hline 
\multicolumn{5}{c}{EW}\\
\hline
C&contac&contact&contactEB &E/KE\\
E/KW&EB/K&EB/KE &EB/KE:&EB/KW\\
EB\_EC&EC &ECL&ECL/C&ECLEC\\
EW & EW/K&EW/K&EW/KE:&EW/KW \\ 
EW/KW:&EW/RS&EW/WTTS&overcontact &W\_URSAE\_MAJ \\
\multicolumn{5}{c}{}\\
\hline
\hline
\multicolumn{5}{c}{ECL}\\
\hline 
CBF&CBH&DBF&DBH &E\\
E/GS &E/PSR&E/RS &E/WD&E/WR\\
EA/EB&EA/EL &EA/EW&EA/SD&EA/SD/RS\\
EA/SD: &EB/EA&EB/EW&EB\_ED\_ESD&EB\_Other \\ 
EC/ESD&EC=ESD&ED/ESD&ESD/EC &ESD/EC/ED\\
ESD=ED&EW/D&EW/DW &EW/DW/RS&EW/DW:\\
EW/EA& \\
\hline

\end{tabular}
\end{table} 


==> DPACP-177_GAIA Cross-match/comparison10.0_class.tex <==

\begin{longtable}{lrrrr}
\caption{\label{table:sourcesPerclass} List of different classes of sources existing in the cross-match catalogue and the number of sources found in the {\tt{primary\_var\_type}} and {\tt{var\_type}} fields with such class. For the field {\tt{var\_type}} if a type is found multiple times for a given source id then it is counted once. The columns {\tt{All}} refer to all sources in our catalogue while {\tt{selection}} only to the cases where {\tt{selection}} flag is true.}\\
\hline \hline 
  & \multicolumn{2}{c}{primary\_var\_type} & \multicolumn{2}{c}{var\_type}\\
 \hline 
Class&All&{\tt{selection}}&All&{\tt{selection}}\\ 
 \hline
 \endfirsthead 
 \hline 
ACEP&600&599&872&871\\ 
ACV&607&607&1414&1414\\ 
ACYG&64&64&75&74\\ 
AGN&5616&4624&24313&23321\\ 
AHB1&2&2&188&188\\ 
ARRD&114&114&170&170\\ 
BCEP&17677&184&19118&1623\\ 
BE&4978&4869&5327&5218\\ 
BHXB&45&45&50&50\\ 
BLAP&14&14&14&14\\ 
BLAZAR&2990&2938&4875&4823\\ 
BLHER&1153&1153&1615&1615\\ 
BLLAC&11&11&650&650\\ 
BY&104699&104695&109833&109829\\ 
BY|ROT&283&283&283&283\\ 
CEP&510&485&961&936\\ 
CP&70&&234&164\\ 
CST&688960&688948&691015&691003\\ 
CTTS&443&443&647&647\\ 
CV&3063&3062&3263&3262\\ 
CW&1265&1265&1596&1596\\ 
DCEP&14601&14430&16115&15944\\ 
DIP&13&13&14&14\\ 
DPV&5&5&26&26\\ 
DQ&244&4&246&5\\ 
DSCT&37656&27605&40766&30715\\ 
DSCT+GDOR&128&128&202&202\\ 
DSCT|SXPHE&8196&8196&8956&8956\\ 
EA&415864&407326&424621&416057\\ 
EB&31796&21819&47003&36898\\ 
ECL&198020&185384&360501&347833\\ 
ELL&28405&27730&29613&28357\\ 
ELM\_ZZA&9&9&10&10\\ 
EP&1053&1053&1155&1155\\ 
EW&482341&477388&537269&531932\\ 
FKCOM&5&5&8&8\\ 
FLARES&9890&854&20567&11528\\ 
FUOR&7&7&13&13\\ 
GALAXY&1746224&1746200&1748871&1748847\\ 
GCAS&2000&2000&2130&2130\\ 
GDOR&1757&1590&2039&1872\\ 
GTTS&13&13&20&20\\ 
GWVIR&782&782&787&787\\ 
HAEBE&30&30&79&79\\ 
HB&147&147&147&147\\ 
HMXB&39&38&41&40\\ 
HOT\_DQ&3&&7&4\\ 
HOT\_DQV&6&6&6&6\\ 
HOT\_ZZA&3&3&3&3\\ 
I&599&553&941&894\\ 
IMTTS&2&2&4&4\\ 
L&15754&15682&21747&21651\\ 
LPV&91816&79980&130165&118323\\ 
LSP&1073&39&1846&812\\ 
M&13597&13304&22028&21596\\ 
\hline
\\
\caption{continued.}\\
\hline 
\hline 
  & \multicolumn{2}{c}{primary\_var\_type} & \multicolumn{2}{c}{var\_type}\\
 \hline 
Class&All&{\tt{selection}}&All&{\tt{selection}}\\ 
 \hline
MCP&2243&2243&3110&3110\\ 
MICROLENSING&2712&113&2740&141\\ 
M|SR&55621&55621&150252&150252\\ 
OMIT&341218&&604313&253449\\ 
OSARG&272570&268951&277507&270351\\ 
PCEB&81&81&81&81\\ 
PPN&13&13&16&16\\ 
PRE\_ELM\_ZZA&10&10&10&10\\ 
PULS\_PMS&5&5&5&5\\ 
PVTEL&14&14&20&20\\ 
QSO&1792477&1639132&1797208&1643863\\ 
R&49&49&71&71\\ 
RAD\_VEL\_VAR&74511&74511&78629&78629\\ 
RCB&75&70&107&102\\ 
ROAM&11&11&12&12\\ 
ROAP&18&18&50&50\\ 
ROT&202126&200830&231056&229760\\ 
RR&94128&122&229514&135000\\ 
RRAB&218723&217115&224482&222874\\ 
RRC&74761&71967&83624&80829\\ 
RRD&5304&5226&7568&7490\\ 
RS&80259&80193&84866&84800\\ 
RV&516&469&696&649\\ 
S&2830&2828&3150&3148\\ 
SARG&4757&&5512&755\\ 
SARV&8&8&8&8\\ 
SB&1571&1571&3256&3256\\ 
SDOR&21&21&23&23\\ 
SN&874&874&875&875\\ 
SOLAR\_LIKE&32341&32341&35836&35836\\ 
SPB&261&202&663&604\\ 
SR&170957&169208&198481&195201\\ 
SRA&190&179&560&548\\ 
SRB&765&735&1230&1193\\ 
SRC&23&22&46&45\\ 
SRD&249&247&393&391\\ 
SRS&7370&7370&8054&8054\\ 
SXARI&23&23&30&30\\ 
SXPHE&92&92&127&127\\ 
SYST&241&241&361&361\\ 
T2CEP&837&730&3173&3064\\ 
TTS&1376&1376&1699&1699\\ 
UV&977&977&1084&1084\\ 
UXOR&57&57&97&97\\ 
V1093HER&10&10&10&10\\ 
V361HYA&57&57&57&57\\ 
V777HER&347&347&348&348\\ 
WARM\_DQ&26&&26&\\ 
WD&448254&&468880&19701\\ 
WR&45&44&46&45\\ 
WTTS&414&414&537&537\\ 
X&42&41&57&56\\ 
YSO&13426&13426&16410&16410\\ 
ZAND&27&27&116&116\\ 
ZZ&10&10&20&20\\ 
ZZA&545&545&554&554\\ 
ZZLEP&13&13&13&13\\ 

 \hline 
 
\end{longtable}

==> DPACP-177_GAIA Cross-match/fieldNames.tex <==
\begin{table}
\centering
\caption{\label{table:catalog_labels} Definition of the fields in the cross-match catalogue. The fields in plural may contain multiple values separeted by ";", thus are regarded as Strings. }
\begin{tabular}{llll}
\hline
\hline
Field name & type & units & Definition\\
\hline
gaia\_dr3\_source\_id& Long&&\textit{Gaia}~DR3 source id\\
non\_gaia\_ids &String&& Identifications from literature catalogues.\\
non\_gaia\_coordinates &String&& Coordinates from literature catalogues.\\
primary\_ra&Double&degrees& Right Ascension from the higher ranked catalogue.\\
primary\_dec&Double&degrees& Declination from the higher ranked catalogue.\\
non\_gaia\_mags&String&& Magnitude(s) from literature\\
synthetic\_distances&Double& & Synthetic astrometric-photometric distance (see Eq.~\ref{eq:rsynth}). \\
primary\_superclass&String& & Generic superclass label corresponding to primary\_var\_type.\\
primary\_var\_type&String& & Variability type from the highest ranked catalogue for a given source.\\ 
var\_types&String& & Variability type(s) from literature, sorted by catalogue rank.\\
original\_var\_types&String&& Original variability (sub)type(s) from literature.\\
original\_alt\_var\_types&String&& Alternative variable type(s) from literature.\\
primary\_period&Double&days&Variability period from the highest ranked catalogue for a given source.\\
periods&String& & Variability period(s) from the literature.\\
other\_periods&String&& Other period(s) from the literature.\\
ref\_epochs&String&& Approximate reference epochs (J2000) of the literature.\\
primary\_catalogue\_label&String& & Label of the highest ranked catalogue for a given source.\\
catalogue\_labels&String&& Label(s) of the literature catalogue(s).\\
references&String&& Reference(s) of the literature.\\
selection&Boolean& & Selection of the most reliable catalogues or classes. \\ 
\hline
\end{tabular}
\end{table}

==> DPACP-177_GAIA Cross-match/overlapsExample.tex <==
\begin{table}
\caption{ Counterparts of \textit{Gaia}~DR3 source\_id 4066039874096072576 in different catalogues, discussed in \ref{subsec:overlaps}. The column {\tt{var\_type}} shows the how it was identified in the different literature catalogues it exists.}
\label{table:missclass}
\centering
\begin{tabular}{llllr}
\hline
\hline
            {\tt{catalogue\_label}}&Id&Coordinates&{\tt{var\_type}}&Period\\
            \hline
            ASASSN\_VAR\_JAYASINGHE\_2019 &  \href{https://asas-sn.osu.edu/variables/252221}{J180253.67-240945.3}&270.72363,-24.16259&SR & 18.31322\\
            COMP\_VAR\_VSX\_2019& \href{https://www.aavso.org/vsx/index.php?view=detail.top&oid=108780}{108780}&270.72383,-24.16267&ECL&2.10904\\
            ASAS\_VAR\_RICHARDS\_2012&180254-2409.7&270.72342,-24.16262&EW&2.10907\\
            INTEGRAL\_VAR\_ALFONSOGARZON\_2012& \href{http://cdsarc.u-strasbg.fr/ftp/cats/J/A+A/548/A79/img/IOMC6842000081.png}{6842000081}& 270.72354,-24.16225&EB&2.10914\\
            \hline
\end{tabular}
\end{table}

==> DPACP-177_GAIA Cross-match/ranking_v10.0.tex <==
\begin{longtable}{l}
\caption{\label{table:rank} Rank-ordered list of literature catalogues.}\\
\hline
\hline
Catalogue  \\
\hline 
\endfirsthead 
GAIA\_CEP\_RIPEPI\_2019\\
GAIA\_DR2\_CLASS\_DSCT\_SXPHE\_SELECTION\\
GAIA\_CEP\_ZAK\_2018\\
GAIA\_GALAXY\_CLEMENTINI\_2020\\
GAIA\_RRL\_GAROFALO\_SELECTION\\
KEPLERGAIA\_BY\_ROT\_DISTEFANO\_2020\\
TESSGAIA\_BY\_ROT\_DISTEFANO\_2020\\
GAIA\_BY\_DISTEFANO\_2019\\
OGLE\_BLAP\_PIETRUKOWICZ\_2017\\
OGLE4\_CEP\_OGLE\_2020\\
OGLE4\_VAR\_OGLE\_2019\\
OGLE4\_BLG\_RRL\_SOSZYNSKI\_2019\\
OGLE4\_GD\_RRL\_SOSZYNSKI\_2019\\
CATALINA\_RRAB\_TORREALBA\_2015\\
OGLE4\_GSEP\_VAR\_SOSZYNSKI\_2012\\
NSVS\_RRAB\_KINEMUCHI\_2006\\
CATALINA\_CSS\_RRAB\_DRAKE\_2013\\
CATALINA\_MLS\_RRAB\_DRAKE\_2013\\
CATALINA\_RRAB\_DRAKE\_2013\\
CATALINA\_SEKBO\_RR\_DRAKE\_2013\\
SDSS\_DSCT\_RR\_SUVEGES\_2012\\
COMP\_OMEGACEN\_RRL\_CLEMENTINI\\
COMP\_M3\_RRL\_CLEMENTINI\\
COMP\_M15\_RRL\_CLEMENTINI\\
COMP\_NGC6388\_RRL\_CLEMENTINI\\
COMP\_NGC6441\_RRL\_CLEMENTINI\\
COMP\_UFD\_RRL\_CLEMENTINI\\
CATALINA\_VAR\_DRAKE\_2014\\
CATALINA\_VAR\_DRAKE\_2017\\
LINEAR\_VAR\_PALAVERSA\_2013\\
SDSS\_PS1\_CATALINA\_RRL\_ABBAS\_2014\\
OGLE4\_SHORTP\_ECL\_SOSZYNSKI\_2014\\
OGLE4\_M54\_VAR\_HAMANOWICZ\_2016\\
GAIA\_ECL\_RYBIZKI\_2018\\
OGLE3\_VAR\_OGLE3\_2012\\
OGLE\_BE\_SABOGAL\_2008\\
OGLE\_BE\_SABOGAL\_2005\\
OGLE\_BE\_MENNICKENT\_2002\\
ASASSN\_DIPPERS\_BREDALL\_2020\\
ASAS3\_MCP\_BERNHARD\_2015\\
ASAS\_KEPLER\_VAR\_PIGULSKI\_2009\\
COMP\_WD\_CORSICO\_2019\\
ASASSN\_VAR\_JAYASINGHE\_2019\\
ASAS\_VAR\_POJMANSKI\_2002\\
ATLAS\_VAR\_HEINZE\_2018\\
COMP\_SPB\_BCEP\_DECAT\_PR\\
IUE\_SPB\_NIEMCZURA\_2003\\
COMP\_GAL\_BCEP\_STANKOV\_2005\\
KEPLER\_DSCT\_GDOR\_BRADLEY\_2015\\
KEPLER\_GDOR\_VANREETH\_2015\\
KEPLER\_DSCT\_GDOR\_DEBOSSCHER\_2011\\
COROT\_DSCT\_GDOR\_SARRO\_2013\\
KEPLER\_DSCT\_GDOR\_UYTTERHOEVEN\_2011\\
2MASS\_GDOR\_ALICAVUS\_2016\\
EROS2\_BEATCEP\_MARQUETTE\_2009\\
ASAS\_SOLAR\_LIKE\_MESSINA\_2010\\
HATNET\_MEMBERS\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010\\
HATNET\_NONMEMBERS\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010\\
KEPLER\_ROAP\_HEY\_2019\\
\hline
\\
\caption{continued.}\\
\hline
\hline 
Catalogue  \\
\hline 
KEPLER\_MCP\_HUMMERICH\_2018\\
TESS\_VAR\_CUNHA\_2019\\
M31\_SEL\_LPV\_MOULD\_2004\\
M33\_CEP\_PELLERIN\_2011\\
GAIA\_M31\_CEP\_GAIA\_2018\\
KEPLER\_FLARES\_COMPILATION\\
KEPLER\_ROT\_REINHOLD\_2015\\
MMT\_M37\_FLARES\_CHANG\_2015\\
GAIA\_ROT\_GAIA\_2017\\
COROT\_ROT\_DEMEDEIROS\_2013\\
NSVS\_VAR\_WILLIAMS\_2004\\
HIP\_VAR\_ESA\_1997\\
SDSS\_CV\_SZKODY\_2011\\
ASAS\_SN\_ASAS\_2019\\
COMP\_CABS\_EKER\_2008\\
COMP\_AP\_RENSON\_2009\\
STEREO\_MAP\_WRAITH\_2012\\
TESS\_ROT\_SIKORA\_2019\\
CAHA\_SOLARLIKE\_MARTINEZ\_2010\\
KEPLER\_ROT\_HOWELL\_2016\\
VVV\_VAR\_BRAGA\_2019\\
IRAS\_LPV\_O\_SUH\_2017\\
IRAS\_LPV\_C\_SUH\_2017\\
IRAS\_LPV\_SUH\_2017\\
IRAS\_LPV\_SIC\_SUH\_2017\\
HALO\_MSR\_MAURON\_2020\\
2MASS\_LPV\_DEMERS\_2007\\
HIPPARCOS\_LPV\_BERGEAT\_2001\\
COMP\_SYST\_BELCZYNSKI\_2000\\
GAIA\_DR2\_SOS\_VARIABLES\_2018\\
GAIA\_DR2\_CLASSIFIER\_VARIABLES\_2018\\
2MASS\_GAIA\_WISE\_SYST\_AKRAS\_2019\\
GAIA\_ICRF2\_QSO\_GAIA\_2017\\
BZCAT\_BLAZARS\_MASSARO\_2015\\
ALMA\_BLAZARS\_BONATO\_2018\\
2WHSP\_BLAZARS\_CHANG\_2017\\
GAIA\_QSO\_GAIA\_CRF3\\
EROSITA\_AGN\_LIU\_2021\\
MILLIQUAS\_QSO\_FLESCH\_2019\\
HMQ\_QSO\_FLESCH\_2015\\
COMP\_ZZ\_NGUYEN\_2020\\
GAIA\_ZZ\_EYER\_2019\\
SOAR\_ZZ\_ROMERO\_2019\\
GALEX\_ZZ\_ROWAN\_2019\\
GAIA\_TRANSIENTS\_ALERTS\_2019\\
COMP\_VAR\_VSX\_2019\\
ZTF\_PERIODIC\_CHEN\_2020\\
IUE\_FKCOM\_BOPP\_1981\\
RAVE\_SOLAR\_LIKE\_ZERJAL\_2017\\
COROT\_SOLAR\_LIKE\_MEDHI\_2007\\
SDSS\_DQWD\_KOESTER\_2019\\
ZTF\_CV\_SZKODY\_2020\\
CATALINA\_CV\_DRAKE\_2014\\
OGLE4\_CV\_2016\_OGLE4\\
COMP\_MICROLENSING\_GAIA\\
GAIA\_GAL\_GAIA\_2018\\
COMP\_BHXRB\_CORRALSANTANA\_2016\\
OGLE4\_GSEP\_CST\_SOSZYNSKI\_2012\\
COMP\_YSO\_VARGA-VEREBELYI\_2020\\
\hline
\\
\caption{continued.}\\
\hline
\hline 
Catalogue  \\
\hline 
COMP\_DSCT\_GDOR\_DEBOSSCHER\_2007\\
DECAM\_VAR\_VIVAS\_2020\\
BULGE\_SOLAR\_LIKE\_DRAKE\_2006\\
ZTF\_CST\_GAIA\_2020\\
TESS\_CST\_GAIA\_2020\\
COMP\_EP\_SOUTHWORTH\_2020\\
PS1\_RRL\_SESAR\_SELECTION\_2017\\
KEPLER\_SHORTP\_SLAWSON\_2011\\
COMP\_XB\_RITTER\_2003\\
COMP\_CV\_RITTER\_2013\\
COMP\_PCB\_RITTER\_2013\\
KEPLER\_ECL\_KIRK\_2016\\
UKST\_LPV\_KUNKEL\_1997\\
SB9\_SB\_POURBAIX\_2004\\
SDSS\_CST\_IVEZIC\_2007\\
LAMOST\_RAD\_VEL\_VAR\_TIAN\_2020\\
GAIA\_WD\_GENTILEFUSILLO\_2019\\
PS1\_RRL\_SESAR\_2017\\
EROS2\_LPV\_SPANO\_2011\\
TRES\_ECL\_DEVOR\_2008\\
KEPLER\_VAR\_DEBOSSCHER\_2011\\
EROS2\_VAR\_KIM\_2014\\
ASAS\_VAR\_RICHARDS\_2012\\
SDSS\_VAR\_IVEZIC\_2007\\
INTEGRAL\_VAR\_ALFONSOGARZON\_2012\\
OGLE4\_MICROLENSING\_OGLE4\_2016\\
HATNET\_COMP\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010\\
OGLE4\_LMC\_CEP\_RR\_OGLE4\_2016\\
OGLE4\_BLG\_CEP\_RR\_OGLE4\_2016\\
OGLE4\_SMC\_CEP\_RR\_OGLE4\_2016\\
OGLE4\_LMC\_ECL\_OGLE4\_2017\\
OGLE4\_SMC\_ECL\_OGLE4\_2017\\
OGLE4\_CEP\_RR\_OGLE\_2016\\
OGLE\_BLG\_EB\_SOSZYNSKI\_2016\\
\hline
\end{longtable}

==> DPACP-177_GAIA Cross-match/refTable_v10.0.tex <==
\begin{longtable}{lll}
\caption{\label{table:catalogList} List of input catalouges used. First column is the {\tt{catalogue\_label}} of the input catalogues used, then the number of objects found in the cross-match follows, and finally references of the catalogue in literature.}\\
\hline 
\hline 
Catalogue\_label & \textnumero ~Objects & Reference \\
\hline 
\endfirsthead 
2MASS\_GAIA\_WISE\_SYST\_AKRAS\_2019&326&{\cite{2019ApJS..240...21A}}\\
2MASS\_GDOR\_ALICAVUS\_2016&51&{\cite{2016MNRAS.458.2307K}}\\
2MASS\_LPV\_DEMERS\_2007&103&{\cite{2007A&A...473..143D}}\\
2WHSP\_BLAZARS\_CHANG\_2017&815&{\cite{2017A&A...598A..17C}}\\
ALMA\_BLAZARS\_BONATO\_2018&1019&{\cite{2018MNRAS.478.1512B}}\\
ASAS3\_MCP\_BERNHARD\_2015&300&{\cite{2015A&A...581A.138B}}\\
ASASSN\_DIPPERS\_BREDALL\_2020&11&{\cite{2020MNRAS.496.3257B}}\\
ASASSN\_VAR\_JAYASINGHE\_2019&345133&{\cite{2019MNRAS.485..961J}}\\
& &{\cite{2014ApJ...788...48S}}\\
& &{\cite{2018MNRAS.477.3145J}}\\
& &{\cite{2019MNRAS.486.1907J}}\\
ASAS\_KEPLER\_VAR\_PIGULSKI\_2009&794&{\cite{2009AcA....59...33P}}\\
ASAS\_SN\_ASAS\_2019&387&{\cite{2014ApJ...788...48S}}\\
ASAS\_SOLAR\_LIKE\_MESSINA\_2010&221&{\cite{2010A&A...520A..15M}}\\
& &{\cite{2011A&A...532A..10M}}\\
ASAS\_VAR\_POJMANSKI\_2002&14994&{\cite{2002AcA....52..397P}}\\
ASAS\_VAR\_RICHARDS\_2012&19117&{\cite{2012ApJS..203...32R}}\\
ATLAS\_VAR\_HEINZE\_2018&356621&{\cite{2018AJ....156..241H}}\\
BULGE\_SOLAR\_LIKE\_DRAKE\_2006&2385&{\cite{2006AJ....131.1044D}}\\
BZCAT\_BLAZARS\_MASSARO\_2015&2686&{\cite{2015Ap&SS.357...75M}}\\
CAHA\_SOLARLIKE\_MARTINEZ\_2010&149&{\cite{2010A&A...520A..79M}}\\
CATALINA\_CSS\_RRAB\_DRAKE\_2013&2007&{\cite{2013ApJ...765..154D}}\\
CATALINA\_CV\_DRAKE\_2014&545&{\cite{2014MNRAS.441.1186D}}\\
CATALINA\_MLS\_RRAB\_DRAKE\_2013&1201&{\cite{2013ApJ...765..154D}}\\
CATALINA\_RRAB\_DRAKE\_2013&12098&{\cite{2013ApJ...763...32D}}\\
CATALINA\_RRAB\_TORREALBA\_2015&10452&{\cite{2015MNRAS.446.2251T}}\\
CATALINA\_SEKBO\_RR\_DRAKE\_2013&550&{\cite{2013ApJ...765..154D}}\\
CATALINA\_VAR\_DRAKE\_2014&46226&{\cite{2014ApJS..213....9D}}\\
CATALINA\_VAR\_DRAKE\_2017&36584&{\cite{2017MNRAS.469.3688D}}\\
COMP\_AP\_RENSON\_2009&3055&{\cite{2009A&A...498..961R}}\\
COMP\_BHXRB\_CORRALSANTANA\_2016&50&{\cite{2016A&A...587A..61C}}\\
COMP\_CABS\_EKER\_2008&260&{\cite{2008MNRAS.389.1722E}}\\
COMP\_CV\_RITTER\_2013&1096&{\cite{2003A&A...404..301R}}\\
COMP\_DSCT\_GDOR\_DEBOSSCHER\_2007&68&{\cite{2007A&A...475.1159D}}\\
COMP\_EP\_SOUTHWORTH\_2020&1048&\cite{2011MNRAS.417.2166S}, \href{https://www.astro.keele.ac.uk/jkt/tepcat/html-catalogue.html}{ URL link}\\
COMP\_GAL\_BCEP\_STANKOV\_2005&41&{\cite{2005ApJS..158..193S}}\\
COMP\_M15\_RRL\_CLEMENTINI&113&{\cite{2008AJ....135.1459C}}\\
COMP\_M3\_RRL\_CLEMENTINI&206&{\cite{2006MNRAS.372.1657B}}\\
COMP\_MICROLENSING\_GAIA&115&Internal\_Microlensing\_Kruszy{\'n}ska\\
COMP\_NGC6388\_RRL\_CLEMENTINI&33&{\cite{2002AJ....124..949P}}\\
& &{\cite{2006AJ....132.1014C}}\\
& &{\cite{2015A&A...573A.103S}}\\
COMP\_NGC6441\_RRL\_CLEMENTINI&43&{\cite{2003AJ....126.1381P}}\\
& &{\cite{2006AJ....132.1014C}}\\
COMP\_OMEGACEN\_RRL\_CLEMENTINI&183&{\cite{2016AJ....152..170B}}\\
COMP\_PCB\_RITTER\_2013&555&{\cite{2003A&A...404..301R}}\\
COMP\_SPB\_BCEP\_DECAT\_PR&69&Internal\_SPB\_BCEP\_DeCat\\
COMP\_SYST\_BELCZYNSKI\_2000&140&{\cite{2000A&AS..146..407B}}\\
COMP\_UFD\_RRL\_CLEMENTINI&64&{\cite{2009MNRAS.398.1757W}}\\
& &{\cite{2006ApJ...649L..83S}}\\
& &{\cite{2012ApJ...756..121M}}\\
& &{\cite{2013ApJ...767...62G}}\\
& &{\cite{2006ApJ...653L.109D}}\\
& &{\cite{2009ApJ...695L..83M}}\\
& &{\cite{2012ApJ...752...42D}}\\
& &{\cite{2013AJ....146...94B}}\\
& &{\cite{2014ApJ...793..135S}}\\
COMP\_VAR\_VSX\_2019&779348&{\cite{2006SASS...25...47W}}\\
\hline
\\
\caption{continued.}\\
\hline 
\hline 
Catalogue\_label & \textnumero ~Objects & Reference \\ 
\hline
COMP\_WD\_CORSICO\_2019&258&{\cite{2019A&ARv..27....7C}}\\
COMP\_XB\_RITTER\_2003&49&{\cite{2003A&A...404..301R}}\\
COMP\_YSO\_VARGA-VEREBELYI\_2020&11036&{\cite{2020IAUS..345..378V}}\\
COMP\_ZZ\_NGUYEN\_2020&31&{\cite{2011ApJ...733L..19D}}\\
& &{\cite{2007ApJS..171..219Q}}\\
& &{\cite{2013MNRAS.436.3573H}}\\
& &{\cite{2013MNRAS.432.1632K}}\\
& &{\cite{2013ApJ...765..102H}}\\
& &{\cite{2012ApJ...750L..28H}}\\
& &{\cite{2010ApJ...720L.159D}}\\
& &{\cite{2014MNRAS.442.2278K}}\\
& &{\cite{2016ApJ...817...27W}}\\
& &{\cite{2009ApJ...690..560N}}\\
& &{\cite{1999ApJ...516..887B}}\\
& &{\cite{2005ApJ...631.1100G}}\\
& &{\cite{2020A&A...638A..82B}}\\
COROT\_DSCT\_GDOR\_SARRO\_2013&712&{\cite{2013A&A...550A.120S}}\\
COROT\_ROT\_DEMEDEIROS\_2013&3862&{\cite{2013A&A...555A..63D}}\\
COROT\_SOLAR\_LIKE\_MEDHI\_2007&174&{\cite{2007A&A...469..713M}}\\
DECAM\_VAR\_VIVAS\_2020&119&{\cite{2020MNRAS.492.1061V}}\\
EROS2\_BEATCEP\_MARQUETTE\_2009&399&{\cite{2009A&A...495..249M}}\\
EROS2\_LPV\_SPANO\_2011&41762&{\cite{2011A&A...536A..60S}}\\
EROS2\_VAR\_KIM\_2014&129954&{\cite{2014A&A...566A..43K}}\\
EROSITA\_AGN\_LIU\_2021&8550&\cite{2021arXiv210614522L}\\
& & \cite{2021arXiv210614523B}\\
& & \cite{2021arXiv210614520S}\\
GAIA\_BY\_DISTEFANO\_2019&24968&Internal\_BY\_Distefano\\
GAIA\_CEP\_RIPEPI\_2019&1339&{\cite{2019A&A...625A..14R}}\\
GAIA\_CEP\_ZAK\_2018&18&Internal\_CEP\_Zak\\
GAIA\_DR2\_CLASSIFIER\_VARIABLES\_2018&360580&{\cite{2018A&A...618A..30H}}\\
GAIA\_DR2\_CLASS\_DSCT\_SXPHE\_SELECTION&1905&Internal\_DSCT\_DeRidder\\
GAIA\_DR2\_SOS\_VARIABLES\_2018&387510&{\cite{2018A&A...618A..30H}}\\
GAIA\_ECL\_RYBIZKI\_2018&2189&{Internal\_ECL\_Rybizki}\\
GAIA\_GALAXY\_CLEMENTINI\_2020&769&{\cite{2019A&A...622A..60C}}\\
GAIA\_GAL\_GAIA\_2018&1748322&{\cite{floisvos}}\\
GAIA\_ICRF2\_QSO\_GAIA\_2017&2079&{\cite{2013yCat.1323....0M}}\\
GAIA\_M31\_CEP\_GAIA\_2018&747&Internal\_CEP\_M31\\
GAIA\_QSO\_GAIA\_CRF3&1614173&\cite{DR3-DPACP-133}\\
GAIA\_ROT\_GAIA\_2017&3725&Internal\_ROT\_Distefano\\
GAIA\_RRL\_GAROFALO\_SELECTION&1569&Internal\_RRL\_Garofalo\\
GAIA\_TRANSIENTS\_ALERTS\_2019&6843&Internal\_Gaia\_Science\_Alerts\\
GAIA\_WD\_GENTILEFUSILLO\_2019&468880&{\cite{2019MNRAS.482.4570G}}\\
GAIA\_ZZ\_EYER\_2019&1461&{\cite{2019arXiv191207659E}}\\
GALEX\_ZZ\_ROWAN\_2019&62&{\cite{2019MNRAS.486.4574R}}\\
HALO\_MSR\_MAURON\_2020&419&{\cite{2019A&A...626A.112M}}\\
HATNET\_COMP\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010&18&{\cite{2010MNRAS.408..475H}}\\
HATNET\_MEMBERS\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010&372&{\cite{2010MNRAS.408..475H}}\\
HATNET\_NONMEMBERS\_PLEIADES\_SOLAR\_LIKE\_HARTMAN\_2010&1724&{\cite{2010MNRAS.408..475H}}\\
HIPPARCOS\_LPV\_BERGEAT\_2001&361&{\cite{2001A&A...369..178B}}\\
HIP\_VAR\_ESA\_1997&48932&{\cite{1997ESASP1200.....E}}\\
HMQ\_QSO\_FLESCH\_2015&294253&{\cite{2015PASA...32...10F}}\\
INTEGRAL\_VAR\_ALFONSOGARZON\_2012&3516&{\cite{2012A&A...548A..79A}}\\
IRAS\_LPV\_C\_SUH\_2017&490&{\cite{2017JKAS...50..131S}}\\
IRAS\_LPV\_O\_SUH\_2017&1498&{\cite{2017JKAS...50..131S}}\\
IRAS\_LPV\_SIC\_SUH\_2017&15&{\cite{2017JKAS...50..131S}}\\
IRAS\_LPV\_SUH\_2017&231&{\cite{2017JKAS...50..131S}}\\
IUE\_FKCOM\_BOPP\_1981&3&{\cite{1981ApJ...247L.131B}}\\
IUE\_SPB\_NIEMCZURA\_2003&40&{\cite{2003A&A...404..689N}}\\
KEPLER\_GAIA\_BY\_ROT\_DISTEFANO\_2020&173&Intenal\_BY\_ROT\_Distefano\\
KEPLER\_DSCT\_GDOR\_BRADLEY\_2015&314&{\cite{2015AJ....149...68B}}\\
\hline
\\
\caption{continued.}\\
\hline 
\hline 
Catalogue\_label & \textnumero ~Objects & Reference \\ 
\hline
KEPLER\_DSCT\_GDOR\_DEBOSSCHER\_2011&1023&{\cite{2011A&A...529A..89D}}\\
KEPLER\_DSCT\_GDOR\_UYTTERHOEVEN\_2011&436&{\cite{2011A&A...534A.125U}}\\
KEPLER\_ECL\_KIRK\_2016&2797&{\cite{2016AJ....151...68K}}\\
KEPLER\_FLARES\_COMPILATION&654&{\cite{2011AJ....141...50W}}\\
& &{\cite{2013ApJS..209....5S}}\\
& &{\cite{2015ApJ...798...92W}}\\
KEPLER\_GDOR\_VANREETH\_2015&68&{\cite{2015ApJS..218...27V}}\\
KEPLER\_MCP\_HUMMERICH\_2018&53&{\cite{2018A&A...619A..98H}}\\
KEPLER\_ROAP\_HEY\_2019&6&{\cite{2019MNRAS.488...18H}}\\
KEPLER\_ROT\_HOWELL\_2016&19&{\cite{2016ApJ...831...27H}}\\
KEPLER\_ROT\_REINHOLD\_2015&19891&{\cite{2015A&A...583A..65R}}\\
KEPLER\_SHORTP\_SLAWSON\_2011&42&{\cite{2011AJ....142..160S}}\\
KEPLER\_VAR\_DEBOSSCHER\_2011&145181&{\cite{2011A&A...529A..89D}}\\
LAMOST\_RAD\_VEL\_VAR\_TIAN\_2020&78629&{\cite{2020ApJS..249...22T}}\\
LINEAR\_VAR\_PALAVERSA\_2013&6851&{\cite{2013AJ....146..101P}}\\
M31\_SEL\_LPV\_MOULD\_2004&442&{\cite{2004ApJS..154..623M}}\\
M33\_CEP\_PELLERIN\_2011&311&{\cite{2011ApJS..193...26P}}\\
MILLIQUAS\_QSO\_FLESCH\_2019&1099699&{\cite{2019arXiv191205614F}}\\
MMT\_M37\_FLARES\_CHANG\_2015&214&{\cite{2015ApJ...814...35C}}\\
NSVS\_RRAB\_KINEMUCHI\_2006&1078&{\cite{2006AJ....132.1202K}}\\
NSVS\_VAR\_WILLIAMS\_2004&5239&{\cite{2004AJ....128.2965W}}\\
OGLE3\_VAR\_OGLE3\_2012&404247&{\cite{2008AcA....58..163S}}\\
& &{\cite{2008AcA....58..293S}}\\
& &{\cite{2009AcA....59....1S}}\\
& &{\cite{2009AcA....59..239S}}\\
& &{\cite{2009AcA....59..335S}}\\
& &{\cite{2010AcA....60....1P}}\\
& &{\cite{2010AcA....60...17S}}\\
& &{\cite{2010AcA....60..179P}}\\
& &{\cite{2010AcA....60...91S}}\\
& &{\cite{2010AcA....60..165S}}\\
& &{\cite{2011AcA....61....1S}}\\
& &{\cite{2011AcA....61..285S}}\\
& &{\cite{2011AcA....61..217S}}\\
& &{\cite{2013AcA....63...21S}}\\
& &{\cite{2013AcA....63..323P}}\\
OGLE4\_BLG\_CEP\_RR\_OGLE4\_2016&36342&{\cite{2017AcA....67..297S}}\\
OGLE4\_BLG\_RRL\_SOSZYNSKI\_2019&65304&{\cite{2019AcA....69..321S}}\\
OGLE4\_CEP\_OGLE\_2020&3692&{\cite{2014AcA....64..177S}}\\
& &{\cite{2015AcA....65..297S}}\\
& &{\cite{2016AcA....66..421P}}\\
& &{\cite{2016AcA....66..131S}}\\
& &{\cite{2017AcA....67..297S}}\\
& &{\cite{2018AcA....68..315U}}\\
& &{\cite{2020AcA....70..101S}}\\
OGLE4\_CEP\_RR\_OGLE\_2016&89511&{\cite{2014AcA....64..177S}}\\
& &{\cite{2015AcA....65..297S}}\\
& &{\cite{2016AcA....66..131S}}\\
& &{\cite{2017AcA....67..297S}}\\
OGLE4\_CV\_2016\_OGLE4&195&{\cite{2015AcA....65..313M}}\\
OGLE4\_GD\_RRL\_SOSZYNSKI\_2019&10008&{\cite{2019AcA....69..321S}}\\
OGLE4\_GSEP\_CST\_SOSZYNSKI\_2012&10495&{\cite{2012AcA....62..219S}}\\
OGLE4\_GSEP\_VAR\_SOSZYNSKI\_2012&6455&{\cite{2012AcA....62..219S}}\\
OGLE4\_LMC\_CEP\_RR\_OGLE4\_2016&43291&{\cite{2015AcA....65..297S}}\\
& &{\cite{2016AcA....66..131S}}\\
OGLE4\_LMC\_ECL\_OGLE4\_2017&38810&{\cite{2016AcA....66..421P}}\\
OGLE4\_M54\_VAR\_HAMANOWICZ\_2016&168&{\cite{2016AcA....66..197H}}\\
OGLE4\_MICROLENSING\_OGLE4\_2016&2707&{\cite{2019ApJS..244...29M}}\\
OGLE4\_SHORTP\_ECL\_SOSZYNSKI\_2014&161&{\cite{2015AcA....65...39S}}\\
\hline
\\
\caption{continued.}\\
\hline 
\hline 
Catalogue\_label & \textnumero ~Objects & Reference \\ 
\hline
OGLE4\_SMC\_CEP\_RR\_OGLE4\_2016&11342&{\cite{2016AcA....66..131S}}\\
& &{\cite{2015AcA....65..297S}}\\
OGLE4\_SMC\_ECL\_OGLE4\_2017&8282&{\cite{2016AcA....66..421P}}\\
OGLE4\_VAR\_OGLE\_2019&496569&{\cite{2014AcA....64..177S}}\\
& &{\cite{2015AcA....65..297S}}\\
& &{\cite{2016AcA....66..421P}}\\
& &{\cite{2016AcA....66..131S}}\\
& &{\cite{2017AcA....67..297S}}\\
& &{\cite{2018AcA....68..315U}}\\
OGLE\_BE\_MENNICKENT\_2002&1002&{\cite{2002A&A...393..887M}}\\
OGLE\_BE\_SABOGAL\_2005&2370&{\cite{2005MNRAS.361.1055S}}\\
OGLE\_BE\_SABOGAL\_2008&1408&{\cite{2008A&A...478..659S}}\\
OGLE\_BLAP\_PIETRUKOWICZ\_2017&14&{\cite{2017NatAs...1E.166P}}\\
OGLE\_BLG\_EB\_SOSZYNSKI\_2016&347267&{\cite{2016AcA....66..405S}}\\
PS1\_RRL\_SESAR\_2017&228876&{\cite{2017AJ....153..204S}}\\
PS1\_RRL\_SESAR\_SELECTION\_2017&60872&{\cite{2017AJ....153..204S}}\\
RAVE\_SOLAR\_LIKE\_ZERJAL\_2017&30830&{\cite{2017ApJ...835...61Z}}\\
SB9\_SB\_POURBAIX\_2004&3256&{\cite{2004A&A...424..727P}}\\
SDSS\_CST\_IVEZIC\_2007&597335&{\cite{2007AJ....134..973I}}\\
SDSS\_CV\_SZKODY\_2011&263&{\cite{2011AJ....142..181S}}\\
SDSS\_DQWD\_KOESTER\_2019&279&{\cite{2019A&A...628A.102K}}\\
SDSS\_DSCT\_RR\_SUVEGES\_2012&259&{\cite{2012MNRAS.424.2528S}}\\
SDSS\_PS1\_CATALINA\_RRL\_ABBAS\_2014&5558&{\cite{2014MNRAS.441.1230A}}\\
SDSS\_VAR\_IVEZIC\_2007&66120&{\cite{2007AJ....134..973I}}\\
SOAR\_ZZ\_ROMERO\_2019&14&{\cite{2019MNRAS.490.1803R}}\\
STEREO\_MAP\_WRAITH\_2012&75&{\cite{2012MNRAS.420..757W}}\\
TESSGAIA\_BY\_ROT\_DISTEFANO\_2020&110&Intenal\_BY\_ROT\_Distefano\\
TESS\_CST\_GAIA\_2020&5072&{\cite{DR3-DPACP-177}}\\
TESS\_ROT\_SIKORA\_2019&131&{\cite{2019MNRAS.487.4695S}}\\
TESS\_VAR\_CUNHA\_2019&51&{\cite{2019MNRAS.487.3523C}}\\
TRES\_ECL\_DEVOR\_2008&714&{\cite{2008AJ....135..850D}}\\
UKST\_LPV\_KUNKEL\_1997&445&{\cite{1997A&AS..122..463K}}\\
VVV\_VAR\_BRAGA\_2019&329&{\cite{2019A&A...625A.151B}}\\
ZTF\_CST\_GAIA\_2020&32053&{\cite{DR3-DPACP-177}}\\
ZTF\_CV\_SZKODY\_2020&251&{\cite{2020AJ....159..198S}}\\
ZTF\_PERIODIC\_CHEN\_2020&746570&{\cite{2020ApJS..249...18C}}\\
\hline
\end{longtable}


==> DPACP-177_GAIA Cross-match/superclassesTable.tex <==
\begin{table}
\centering
\caption{\label{table:sourcesPerSuperclass} List of available types of {\tt{primary\_superclass}}. The second column shows the {\tt{primary\_var\_types}} that contribute to this {\tt{primary\_superclass}}. The last two columns give the number of sources for each of  {\tt{primary\_superclass}} in the full catalogue ({\tt{All}}) and when the {\tt{selection}} flag is true.}
\begin{tabular}{llrr}
\hline
\hline
{\tt{primary\_superclass}}&{\tt{primary\_var\_types}}&All&{\tt{selection}}\\ 
\hline 
ACYG&ACYG&64&64\\ 
AGN&AGN, BLAZAR, BLLAC, QSO&1801094&1646705\\ 
AHB1&AHB1&2&2\\ 
BCEP&BCEP&17677&184\\ 
BE&BE&4978&4869\\ 
BHXB&BHXB&45&45\\ 
BLAP&BLAP&14&14\\ 
CEP&ACEP, BLHER, CEP, CW, DCEP, RV, T2CEP&19482&19131\\ 
CP&ACV, CP, MCP, ROAM, ROAP&2949&2879\\ 
CST&CST, DQ, HOT\_DQ, WARM\_DQ, WD&1137487&688952\\ 
CV&CV, SN&3937&3936\\ 
DPV&DPV&5&5\\ 
DSCT&DSCT&37656&27605\\ 
DSCT+GDOR&DSCT+GDOR&128&128\\ 
DSCT|SXPHE&DSCT|SXPHE&8196&8196\\ 
ECL&EA, EB, ECL, EW&1128021&1091917\\ 
ELL&ELL&28405&27730\\ 
EP&EP&1053&1053\\ 
FKCOM&FKCOM&5&5\\ 
GALAXY&GALAXY&1746224&1746200\\ 
GCAS&GCAS&2000&2000\\ 
GDOR&GDOR&1757&1590\\ 
HB&HB&147&147\\ 
HMXB&HMXB&39&38\\ 
I&I&599&553\\ 
L&L&15754&15682\\ 
LPV& LPV, LSP, M, M|SR, OSARG, SARG, SR, SRA, SRB, SRC,&618988&595656\\ 
& SRD, SRS&&\\ 
MICROLENSING&MICROLENSING&2712&113\\ 
OMIT&OMIT&341218&null\\ 
PCEB&PCEB&81&81\\ 
PPN&PPN&13&13\\ 
PVTEL&PVTEL&14&14\\ 
R&R&49&49\\ 
RAD\_VEL\_VAR&RAD\_VEL\_VAR&74511&74511\\ 
RCB&RCB&75&70\\ 
RR&ARRD,RR,RRAB,RRC,RRD&393030&294544\\ 
S&S&2830&2828\\ 
SARV&SARV&8&8\\ 
SB&SB&1571&1571\\ 
SDOR&SDOR&21&21\\ 
SOLAR\_LIKE&BY, BY|ROT, FLARES, ROT, RS, SOLAR\_LIKE, UV&430575&420173\\ 
SPB&SPB&261&202\\ 
SXARI&SXARI&23&23\\ 
SXPHE&SXPHE&92&92\\ 
SYST&SYST, ZAND&268&268\\ 
V1093HER&V1093HER&10&10\\ 
V361HYA&V361HYA&57&57\\ 
WR&WR&45&44\\ 
X&X&42&41\\ 
YSO&CTTS, DIP, FUOR, GTTS, HAEBE, IMTTS, PULS\_PMS, TTS,&15786&15786\\ 
&UXOR, WTTS, YSO&&\\ 
ZZ&ELM\_ZZA, GWVIR, HOT\_DQV, HOT\_ZZA, PRE\_ELM\_ZZA,&1712&1712\\ 
&V777HER, ZZ, ZZA&&\\ 
ZZLEP&ZZLEP&13&13\\ 
\hline \\ 
\end{tabular}
\end{table} 
